Decision Making in Changing Environments: Robustness, Query-Based Learning, and Differential Privacy

We study the problem of interactive decision making in which the underlying environment changes over time subject to given constraints. We propose a framework, which we call \textit{hybrid Decision Making with Structured Observations} (hybrid DMSO), that provides an interpolation between the stochastic and adversarial settings of decision making. Within this framework, we can analyze local differentially private (LDP) decision making, query-based learning (in particular, SQ learning), and robust and smooth decision making under the same umbrella, deriving upper and lower bounds based on variants of the Decision-Estimation Coefficient (DEC). We further establish strong connections between the DEC's behavior, the SQ dimension, local minimax complexity, learnability, and joint differential privacy. To showcase the framework's power, we provide new results for contextual bandits under the LDP constraint.

==> appdx_CBs-proof.tex <==
\section{Proofs for}

\subsection{Contextual DMSO}



In the contextual DMSO framework~\citep{foster2021statistical}, we adopt the following protocol for $T$ rounds. For each $t=1,\cdots,T$:
\newcommand{\tz}{\Tilde{z}}
\begin{itemize}
  \setlength{\parskip}{2pt}
    \item The learner selects a decision $\pi^t\in \Pi$ and a privacy mechanism $\pr^t\in\Pc$, where $\Pi$ is the decision space.
    \item The $t$-th user with context $x^t\in\cX$ receives 
    $(\pi^t,\pr^t)$, executes $\pi^t$, receives an observation $z^t=(x^t,\tz^t)$ sampled via $\tz^t\sim \Mscxt(\pi^t,x^t)$. 
    \item The user generates a noisy observation $o^t\in\cO$ via $o^t\sim \pr^t(\cdot|z^t)$ and sends it to the server.
\end{itemize}
The underlying model $\Mscxt: \Pi\times\cX\to\DZ$ is formally a conditional distribution of the observation $\tz$ on decision $\pi$ and context $x$. The learner is still assumed to have access to a known \emph{contextual} model class $\cMcxt\subseteq (\Pi\times \cX\to\Delta(\cZ))$ containing $\Mscxt$. \cfn{I guess this formulation is too abstract...}


\newcommandx{\Rew}[1][1=M]{\mathsf{R}^M}
In the formulation above, we do not assume any prior knowledge on the context sequence $(x^1,\cdots,x^T)$, and the context $x^t$ can be generated in an adversarial fashion. In this paper, we mainly focus on the following (adversarial) contextual bandits problem (\CB).
\begin{example}[Contextual bandits]\label{CB}
A \CB~problem is specified by a context space $\cX$, action space $\cA$, and a value function class $\cF\subseteq (\cX\times \cA\to[-1,1])$. The decision space $\Pi=(\cX\to\cA)$, i.e., the set of all function $\pi:\cX\to \cA$, and the observation space $\cZ=\cX\times\cA\times[-1,1]$. For each value function $f\in\cF$, it corresponds to a model $M_f\in\cMcxt$, and $\tz\sim M_f(\pi,x)$ is generated as
\begin{align*}
    \tz=(a,r), \qquad a=\pi(x), r\sim \Bern{ f(x,a) },
\end{align*}
where $\Bern{b}$ is the Bernoulli distribution on $\set{-1,1}$ with mean $b$.\footnote{We assume the rewards are Bernoulli without any loss of generality.}
\end{example}







==> appdx_reduction.tex <==

In this section, we briefly review the definitions of DECs in \citet{foster2021statistical,foster2023tight} and the general DEC lower bounds provided in \citet{chen2024beyond} (\cref{appdx:DEC-general-lower}). We then provide the proof of \cref{thm:pdec-lin-lower} in \cref{appdx:p-dec-q}, following the approach of \citet{chen2024beyond}.

\paragraph{Constrained DECs}
Fix a DMSO problem class $(\cM,\Pi)$. For any reference model $\oM: \Pi\to \Delta(\cO)$ (not necessarily in $\cM$), we define the constrained DECs~\citep{foster2021statistical} as follows. For each $\eps>0$,
\begin{align}\label{def:p-dec-c}
    \pdecc_{\eps}(\cM,\oM)\defeq&~ \infpq \sup_{M\in\cM}\constr{ \EE_{\pi\sim p}[\LM{\pi}] }{ \EE_{\pi\sim q} \DH{ M(\pi), \oM(\pi) }\leq \eps^2 },
\end{align}
\begin{align}\label{def:r-dec-c}
    \rdecc_{\eps}(\cM,\oM)\defeq&~ \infp\sup_{M\in\cM}\constr{ \EE_{\pi\sim p}[\LM{\pi}] }{ \EE_{\pi\sim p} \DH{ M(\pi), \oM(\pi) }\leq \eps^2 },
\end{align}
and we further define
\begin{align}
    \pdecc_{\eps}(\cM)=\sup_{\oM\in\coM} \pdecc_{\eps}(\cM,\oM),
    \quad
    \rdecc_{\eps}(\cM)=\sup_{\oM\in\coM} \rdecc_{\eps}(\cMp,\oM).
\end{align}






\newcommandx{\hgm}[3][1=M,2=\delta]{\widehat{L}_{#2}(#1,#3)}









\subsection{LDP DMSO and the General DMSO framework}\label{appdx:DEC-general-lower}


\newcommand{\ext}[1]{{#1}^{\sharp}}
\newcommand{\tPi}{\ext{\Pi}}
\newcommand{\tcM}{\ext{\cM}}
\newcommand{\tM}{\ext{M}}
\newcommand{\talg}{\ext{\alg}}
\newcommand{\tpi}{\bpi}
Given a model class $\cM \subseteq (\Pi\to \DZ)$ and a class of private channels $\Pc\subseteq \Pcp$, we consider the ``enlarged'' decision space $\tPi=\Pi\times\Pc$. Each model $M\in\cM$ corresponds to a model $\tM: \tPi\to \DO$, given as follows:
\begin{align*}
    \text{For each }\bpi=(\pi,\pr)\in\tPi, \qquad &~\tM(\bpi)=\pr\circ M(\pi)\in\DO, \\
    &~ \gm[\tM](\bpi)=\LM{\pi}.
\end{align*}
We then consider the corresponding model class $\tcM\subseteq (\tPi\to \DO)$ given by
\begin{align*}
    \tcM=\sset{ \tM: M\in\cM }.
\end{align*}

\textbf{Claim.} Suppose that $\Pc=\Pcp$, i.e. it is the class of all \pLDP~channels. Then learning $(\cM,\Pi)$ under \pLDP~is equivalent to learning $(\tcM,\tPi)$. 

More specifically, any algorithm $\alg$ for the learning problem $(\tcM,\tPi)$, $\alg$ is a \pLDP~algorithm for $(\cM,\Pi)$, and vice versa. In other words, there is a one-to-one correspondence between
\begin{align*}
    \sset{\text{$T$-round algorithm for learning }(\tcM,\tPi)} \leftrightarrow 
    \sset{\text{$T$-round \pLDP~algorithm for learning }(\cM,\Pi)}.
\end{align*}



Therefore, proving lower (upper) bounds for LDP learning $(\cM,\Pi)$ is equivalent to proving lower (upper) bounds for learning $(\tcM,\tPi)$. Indeed, it follows immediately from \cref{prop:pLDP} that the constrained DEC of $\tcM$ is equivalent to the private DEC of $\cM$.

\begin{lemma}\label{lem:decc-to-lin}
For PAC learning, it holds that 
\begin{align*}
    \pdecl_{c_0\eps/\alpha}(\cM)\leq&~ 
    \pdecc_{\eps}(\tcM) \leq 
    \pdecl_{c_1\eps/\alpha}(\cM), \quad\forall \eps>0,
\end{align*}
where $c_0, c_1>0$ are universal constants. 
Similar, for \rewmax~problem class $\cM$, it holds that
\begin{align*}
    \rdecl_{c_0\eps/\alpha}(\cM)\leq&~ 
    \rdecc_{\eps}(\tcM) \leq 
    \rdecl_{c_1\eps/\alpha}(\cM), \quad\forall \eps>0.
\end{align*}
\end{lemma}















\subsubsection{Proof of \cref{thm:pdec-lin-lower} and \cref{thm:rdec-lin-lower}}

In this section, we derive the private DEC lower bounds from the results of~\citet{chen2024beyond}. A self-contained proof of \cref{thm:pdec-lin-lower} is presented in \cref{appdx:p-dec-q}.



We first summarize the results of \citet[?]{chen2024beyond} as follows.
\begin{theorem}[Constrained DEC lower bounds]\label{cor:decc-lower-pr}
Let $T\geq 1$, and $\alg$ is a $T$-round algorithm for $\tcM$. Suppose that for any model $M\in\cM$, the risk function takes form $\LM{\pi}=\Vmm-\Vm(\pi)$. Further, suppose that for any decision $\pi\in\Pi$, there exists a channel $\pr_\pi\in\Pc$, such that for $\bpi=(\pi,\pr_\pi)\in\tPi$, 
\begin{align}\label{eqn:lip-rew-pr}
    \abs{ \Vm(\pi)-\Vm[\oM](\pi) }\leq \Lipr\dH\paren{\ext{M}(\bpi),\ext{\oM}(\bpi)},\qquad \forall M\in\cM, \oM\in\coM.
\end{align}
Then, the following holds.

(1) PAC lower bound: there exists $\tM\in\tcM$ such that under $\PP\sups{\tM,\alg}$,
\begin{align*}
    \riskdm(T)\geq \pdecc_{\ueps(T)}(\tcM)-C\Lipr\ueps(T), \qquad\text{with probability at least }\frac14,
\end{align*}
where $C, c>0$ are universal constants, and $\ueps(T)=\frac{c}{\sqrt{T}}$.

(2) Regret lower bound: if $M$ is a no-regret learning problem class, there exists $\tM\in\tcM$ such that under $\PP\sups{\tM,\alg}$,
\begin{align*}
    \frac1T\regdm(T)\geq \frac12\rdecc_{\ueps(T)}(\tcM)-C\Lipr\ueps(T), \qquad\text{with probability at least }\frac14.
\end{align*}
\end{theorem}

Under \rewt, the assumption \cref{eqn:lip-rew-pr} is satisfied automatically for the class $\Pc=\Pcp$. To see this, for any decision $\pi\in\Pi,$ we consider the following binary channel (\cref{example:binary-pr}):
\begin{align*}
    \pr_\pi(+1|z)=\frac{1+c R(z,\pi)}{2}, \qquad 
    \pr_\pi(-1|z)=\frac{1-c R(z, \pi)}{2},
\end{align*}
where $\ca=1-\eai$. Then we know \eqref{eqn:lip-rew-pr} holds with $\Lipr=\frac{\sqrt{2}}{c}\leq \bigO{\frac1\alpha}$.
Therefore, combining \cref{cor:decc-lower-pr} with \cref{lem:decc-to-lin} completes the proof of \cref{thm:pdec-lin-lower} and \cref{thm:rdec-lin-lower}. 
\qed

\subsection{Additional details on the \pDEC~lower bound and proof of \cref{thm:pdec-lin-lower}}\label{appdx:p-dec-q}

In this section, we provide a self-contained proof of \cref{thm:pdec-lin-lower}, to illustrate how we can prove the \pDEC~lower bound without going through the reduction in \cref{appdx:DEC-general-lower}.
The proof is based on the following quantile-based DEC proposed by \citep{chen2024beyond}. We also note that the \rDEC~lower bound can be derived similarly, following \citet[?]{chen2024beyond}.

Given model class $\cM$, for each $\eps>0$ and $\delta\in[0,1]$, we define the quantile-based \pDEC~as (slightly abusing the notation)
\begin{align}\label{def:p-dec-q-lin}
    \pdecql_{\eps,\delta}(\cM,\oM)\defeq \infpql\sup_{M\in\cM}\constr{ \hgm{p} }{ \EE_{(\pi,\lf)\sim q}\Dl^2( M(\pi),\oM(\pi) )\leq \eps^2 },
\end{align}
where $\hgm{p}$ is the \emph{$\delta$-quantile loss} of $p$, defined as
\begin{align*}
    \hgm{p}=\sup_{\Delta\geq 0}\set{\Delta: \PP_{\pi\sim q}(\LM{\pi}\geq \Delta)\geq \delta }.
\end{align*}
We also denote $\pdecql_{\eps,\delta}(\cM)\defeq \sup_{\oM\in\coM} \pdecql_{\eps,\delta}(\cM,\oM)$.
By definition, the quantile-based \pDEC~is always bounded by the original \pDEC:
\begin{align}\label{eqn:dec-q-to-c-trivial}
    \pdecql_{\eps}(\cM,\oM)-\delta\leq \pdecql_{\eps,\delta}(\cM,\oM)\leq \delta^{-1}\pdecql_{\eps}(\cM,\oM).
\end{align}
However, such a conversion can be loose in general.

The advantage of considering the quantile \pDEC is that it provides lower bounds for private PAC learning beyond \rewt~(proof in \cref{appdx:proof-p-dec-q-lin-lower}).
\begin{proposition}[Quantile-based \pDEC~lower bound]\label{prop:p-dec-q-lin-lower}
For any $T\geq 1$ and constant $\delta\in[0,1)$, we denote $\ueps(T)\defeq \frac{1}{(\ea-1)}\sqrt{\frac{\delta}{2T}}$. Then, for any $T$-round \pLDP~algorithm $\alg$, there exists $\Ms\in\cM$ such that under $\PP\sups{\Ms,\alg}$,
\begin{align*}
    \riskdm(T)\geq \pdecql_{\ueps(T),\delta}(\cM),\qquad\text{with probability at least $\delta/2$.}
\end{align*}
\end{proposition}

Further, under \rewt, we can relate quantile-based \pDEC~to the original \pDEC~following \citet[Proposition ?]{chen2024beyond}.

\begin{proposition}\label{prop:p-dec-q-lin-to-c}
Suppose that $\cM$ is a \rewmax~problem class. Then, for any parameter $\eps>0, \delta\in[0,1)$, it holds that
\begin{align*}
    \pdecl_{\eps}(\cM)\leq \pdecql_{\sqrt{2}\eps,\delta}(\cM)+\frac{2\sqrt{2}\eps}{1-\delta}.
\end{align*}
\end{proposition}

Combining \cref{prop:p-dec-q-lin-lower} with \cref{prop:p-dec-q-lin-to-c} completes the proof of \cref{thm:pdec-lin-lower}. Further, for any general problem class $\cM$, we also have the following weaker lower bound with \pDEC.
\begin{corollary}\label{cor:pdec-lin-lower-weak}
For any $T\geq 1$ and constant $\delta\in[0,1)$, we denote $\ueps(T)\defeq \frac{1}{(\ea-1)}\sqrt{\frac{\delta}{2T}}$. Then, for any $T$-round \pLDP~algorithm $\alg$, 
\begin{align*}
    \sup_{M\in\cM}\Emalg{\riskdm(T)}\geq \pdecl_{\ueps(T)}(\cM)-\delta.
\end{align*}
\end{corollary}

\paragraph{Better lower bound under stronger condition}
The \pDEC~lower bound (\cref{thm:pdec-lin-lower}) involves a term $-\ueps(T)$, which can be undesirable in some scenarios. However, this factor can be in fact removed if the lower bound can be ``proven using the standard two-point method'' (\cref{asmp:gen-tri}). %
In addition to the above conversion, we also prove that under a different setting, the quantile DEC can also be lower bounded, without subtracting a factor of $\eps$. 
\begin{assumption}\label{asmp:gen-tri}
For some universal constant $C_1, C_2$, it holds that for any models $M, M'\in\cM$, any decision $\pi\in\Pi$,
\begin{align*}
    \LM[M']{\pi}\leq C_1 \LM{\pi}+C_2\inf_{\pi'}\paren{ \LM{\pi'}+\LM[M']{\pi'} }.
\end{align*}
\end{assumption}

For example, when $\LM{\pi}=\nrm{ \pi-\pim }$ for certain norm structure $\nrm{\cdot}$ over $\Pi$, \cref{asmp:gen-tri} holds with $C_1=C_2=1$. Therefore, \cref{asmp:gen-tri} can be viewed as a \emph{generalized} norm structure on the risk functional $\gm$.

\begin{proposition}
\label{prop:p-dec-c-lower-tri}
Suppose that \cref{asmp:gen-tri} holds. For any $T$-round \pLDP~algorithm $\alg$, there exists $\Ms\in\cM$ such that under $\PP\sups{\Ms,\alg}$,
\begin{align*}
    \riskdm(T)\geq \frac{1}{2C_2}\pdecl_{\ueps(T)}(\cM),\qquad\text{with probability at least }\frac14,
\end{align*}
where $\ueps(T)=\frac{1}{(\ea-1)}\sqrt{\frac{\delta}{2T}}$.
\end{proposition}

\subsection{Proof of \cref{prop:p-dec-q-lin-lower}}\label{appdx:proof-p-dec-q-lin-lower}
\newcommand{\tq}{\Tilde{q}}

Following \citet{foster2021statistical}, we first introduce some notations.

Recall that an algorithm $\alg = \set{q\ind{t}}_{t\in [T]}\cup\set{p}$ is specified by a sequence of mappings, where the $t$-th mapping $q\ind{t}(\cdot\mid{}\Hy\ind{t-1})$ specifies the distribution of $(\pi\ind{t},\pr\ind{t})$ based on the history $\Hy\ind{t-1}$, and the final map $p(\cdot \mid{} \Hy\ind{T})$ specifies the distribution of the \emph{output policy} $\pihat$ based on $\Hy\ind{T}$. Therefore, for any model $M$, we define
\begin{align}\label{def:pM-qM}
q_{M,\alg}=\Emalg{ \frac{1}{T} \sum_{t=1}^{T} q\ind{t}(\cdot|\cH\ind{t-1}) }\in \DPP, \quad 
p_{M,\alg}=\Emalg{p(\cH\ind{T})} \in \DPi,
\end{align}
The distribution $q_{M,\alg}$ is the expected distribution of the average profile $(\pi\ind{1},\pr\ind{1},\cdots,\pi\ind{T},\pr\ind{T})$, and $p_{M,\alg}$ is the expected distribution of the output policy $\hpi$. 

Using the chain rule of KL divergence, for any model $M, \oM$,
\begin{align*}
\KLd{\PP\sups{\oM,\alg}}{\PP\sups{M,\alg}}  
=&~ \EE^{\oM,\alg}\brac{ \sum_{t=1}^T \KLd{ \pr\ind{t}\circ M(\pi\ind{t}) }{ \pr\ind{t}\circ M(\pi\ind{t}) } } \\
=&~ T\cdot \EE_{(\pi,\pr)\sim q_{\oM,\alg}} \KLd{ \pr\circ \oM(\pi) }{ \pr\circ M(\pi) }.
\end{align*}
Further, by \cref{prop:pLDP}, for any \pLDP~channel $\pr$, there exists a distribution $\tq_\pr\in\DL$ such that
\begin{align*}
    \KLd{ \pr\circ \PP_1 }{ \pr\circ\PP_2 }\leq (\ea-1)^2\EE_{\lf\sim \tq_\pr} \Dl^2(\PP_1, \PP_2).
\end{align*}

Therefore, for any model $M\in\cM$, we define $\tq_{M,\alg}\in\DPL$ to be the distribution of $(\pi,\lf)$, where $(\pi,\pr)\sim q_{M,\alg}$, and $\lf\sim \tq_{\pr}$. Then, our argument above gives
\begin{align}\label{eqn:KL-chain}
\KLd{\PP\sups{\oM,\alg}}{\PP\sups{M,\alg}}  
\leq (\ea-1)^2 T\cdot \EE_{(\pi,\lf)\sim \tq_{\oM,\alg}} \Dl^2( M(\pi) , \oM(\pi) ).
\end{align}
With this chain rule, we now present the proof of \cref{prop:p-dec-q-lin-lower}~(which is essentially following the analysis in \citet{chen2024beyond}).

\paragraph{Proof of \cref{prop:p-dec-q-lin-lower}}
We abbreviate $\eps=\ueps(T)$. Fix a $\Delta<\pdecql_{\eps,\delta}(\cM)$, and then there exists $\oM$ such that $\Delta<\pdecq_{\eps,\delta}(\cM,\oM)$. Hence, by the definition \cref{def:p-dec-q-lin}, we know that
\begin{align*}
    \Delta<\sup_{M\in\cM}\constr{ \hgm{p_{\oM,\alg}} }{ \EE_{(\pi,\lf)\sim \tq_{\oM,\alg}}\Dl^2( M(\pi) , \oM(\pi) )\leq \eps^2 }.
\end{align*}
Therefore, there exists $M\in\cM$ such that
\begin{align*}
    \EE_{(\pi,\lf)\sim \tq_{\oM,\alg}}\Dl^2( M(\pi) , \oM(\pi) )\leq \eps^2, \qquad
    \PP_{\pi\sim p_{\oM,\alg}}(\LM{\pi}>\Delta)\geq \delta.
\end{align*}
By \cref{eqn:KL-chain}, we know
\begin{align*}
    \KLd{\PP\sups{\oM,\alg}}{\PP\sups{M,\alg}} \leq (\ea-1)^2T\eps^2.
\end{align*}
By data-processing inequality, we have
\begin{align*}
    \DTV{ p_{\oM,\alg}, p_{M,\alg} } \leq \DTV{ \PP\sups{\oM,\alg}, \PP\sups{M,\alg} } \leq \sqrt{\frac{1}{2}(\ea-1)^2T\eps^2}.
\end{align*}
Therefore, combining the inequalities above, we have
\begin{align*}
    p_{M,\alg}(\pi: \LM{\pi}> \Delta )\geq  p_{\oM,\alg}(\pi: \LM{\pi}> \Delta )-\sqrt{\frac{1}{2}(\ea-1)^2T\eps^2}\geq \frac{\delta}{2}.
\end{align*}
By the definition of $p_{M,\alg}$, this gives $\PP\sups{M,\alg}\paren{ \LM{\hpi}> \Delta }\geq \frac\delta2$.
Letting $\Delta\to \pdecq_{\eps,\delta}(\cM)$ completes the proof.
\qed

\subsection{Proof of \cref{prop:p-dec-q-lin-to-c}}

We only need to prove that for $\eps\in[0,1]$,
\begin{align*}
    \pdecql_{\eps,1/2}(\cM)\geq \frac{1}{2C_2}\pdecl_{\eps}(\cM).
\end{align*}

Fix a reference model $\oM$ and let $\Delta_0>\pdecq_{\eps,\delta}(\cM,\oM)$. Then there exists $p\in\DDD, q\in\DPi$ such that
\begin{align*}
    \sup_{M\in\cM}\constr{ \hgm{p} }{ \EE_{(\pi,\lf)\sim q}\Dl^2( M(\pi) , \oM(\pi) )\leq \eps^2 }< \Delta_0.
\end{align*}
Therefore, we denote $\cM_{q,\eps}(\oM)\defeq \set{ M\in\cM: \EE_{(\pi,\lf)\sim q}\Dl^2( M(\pi) , \oM(\pi) )\leq \eps^2 }$, and it holds that
\begin{align*}
    \PP_{\pi\sim q}(\LM{\pi}\leq \Delta_0)\geq 1-\delta, \qquad \forall M\in\cM_{q,\eps}(\oM).
\end{align*}
If the constrained set $\cM_{q,\eps}(\oM)$ is empty, then we immediately have $\pdecc_{\eps}(\cM,\oM)=0$, and the proof is completed. Therefore, in the following we may assume $\cM_{q,\eps}(\oM)$ is non-empty, and fix a model $\hM\in \cM_{q,\eps}(\oM)$.

Notice that for any model $M\in \cM_{q,\eps}(\oM)$, we have
\begin{align*}
    \PP_{\pi\sim q}(\LM{\pi}\leq \Delta_0, \LM[\hM]{\pi}\leq \Delta_0)\geq 1-2\delta>0,
\end{align*}
and hence
\begin{align*}
    \inf_\pi\paren{ \LM{\pi}+\LM[\hM]{\pi} }\leq 2\Delta_0.
\end{align*}
Therefore, \cref{asmp:gen-tri} implies that
\begin{align*}
    \LM[M]{\pi}\leq C_1\LM[\hM]{\pi}+2C_2\Delta_0, \qquad \forall M\in \cM_{q,\eps}(\oM).
\end{align*}

Hence, we can take any $\pis$ such that $\LM[\hM]{\pis}=0$, and let $p_0\in\DPi$ be supported on $\pis$. Then, $(p_0,q)$ certifies that
\begin{align*}
    \pdecc_{\eps}(\cM,\oM)\leq \sup_{M\in\cM}\constr{ \LM{\pis} }{ \EE_{(\pi,\lf)\sim q}\Dl^2( M(\pi) , \oM(\pi) ) \leq \eps^2 } \leq 2C_2\Delta_0.
\end{align*}
Letting $\Delta_0\to\pdecql_{\eps,\delta}(\cM,\oM)$ yields $\pdecl_{\eps}(\cM,\oM)\leq 2C_2 \cdot \pdecql_{\eps,\delta}(\cM,\oM)$, which is the desired result.
\qed

